Featurising Pixels from Dynamic 3D Scenes with Linear In-Context Learners

One of the most exciting applications of vision models involve pixel-level reasoning. Despite the abundance of vision foundation models, we still lack representations that effectively embed spatio-temporal properties of visual scenes at the pixel level. Existing frameworks either train on image-based pretext tasks, which do not account for dynamic elements, or on video sequences for action-level reasoning, which does not scale to dense pixel-level prediction. We present a framework that learns pixel-accurate feature descriptors from videos, LILA. The core element of our training framework is linear in-context learning. LILA leverages spatio-temporal cue maps -- depth and motion -- estimated with off-the-shelf networks. Despite the noisy nature of those cues, LILA trains effectively on uncurated video datasets, embedding semantic and geometric properties in a temporally consistent manner. We demonstrate compelling empirical benefits of the learned representation across a diverse suite of vision tasks: video object segmentation, surface normal estimation and semantic segmentation.

==> preamble.tex <==


\usepackage{microtype}








\usepackage{graphicx}
\usepackage{bbding}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{microtype}
\usepackage[percent]{overpic}

\usepackage{etoolbox,siunitx}
\robustify\bfseries
\sisetup{detect-all = true}


\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\usepackage{xcolor}
\usepackage{colortbl}
\definecolor{azure}{rgb}{0.95, 0.95, 1.0}

\newcommand{\tabmark}[2]{%
  \phantomsubcaption\label{#1}%
  \subref*{#1}~#2%
}

\newcommand*{\inparagraph}[1]{\noindent\textbf{#1}\hspace{0.5em}}
\newcommand{\emdash}{\unskip\nobreak\thinspace---\thinspace\ignorespaces}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\prelim}[1]{{\color{blue}#1}}

\newcommand{\projectwebsite}[1]{%
  \begingroup
  \let\thefootnote\relax
  \footnotetext{Project website: \url{#1}}%
  \endgroup
}

\newcommand{\oursName}{LILA\@\xspace}
\newcommand{\supp}{supp.\ material\@\xspace}
\newcommand{\leftPad}{\: +\,}
\newcommand{\JF}{$\mathcal{JF}$\@\xspace}

\newcommand{\hide}[1]{\textbf{\color{blue}H: #1}}
\newcommand{\martin}[1]{\textcolor[rgb]{0,0,1}{#1}}

\definecolor{cb-blue}{HTML}{0072B2}
\definecolor{cb-orange}{HTML}{D55E00}

\newcommand{\diffp}[1]{\textcolor{cb-blue}{\scriptsize (+#1)}}
\newcommand{\diffn}[1]{\textcolor{cb-orange}{\scriptsize (#1)}}
\newcommand{\diffz}[1]{\textcolor{gray}{\scriptsize (#1)}}


\newcommand{\xmark}{\textcolor{red}{$\boldsymbol{\times}$}}
\newcommand{\concat}{\|}
\newcommand{\cxt}{0}
\newcommand{\qry}{\Delta}

\newcommand{\FixedHeader}[1]{%
    \parbox[b][0.8em][t]{\linewidth}{\centering\footnotesize #1}%
}

\newcommand{\FancyBlueRightArrow}{%
    \textcolor{violet}{$\:\blacktriangleright\:$}
}

